Adversarial Attacks and Defenses on Graphs: A Review, A Tool and Empirical Studies

Deep neural networks (DNNs) have achieved significant performance in various tasks. However, recent studies have shown that DNNs can be easily fooled by small perturbation on the input, called adversarial attacks. As the extensions of DNNs to graphs, Graph Neural Networks (GNNs) have been demonstrated to inherit this vulnerability. Adversary can mislead GNNs to give wrong predictions by modifying the graph structure such as manipulating a few edges. This vulnerability has arisen tremendous concerns for adapting GNNs in safety-critical applications and has attracted increasing research attention in recent years. Thus, it is necessary and timely to provide a comprehensive overview of existing graph adversarial attacks and the countermeasures. In this survey, we categorize existing attacks and defenses, and review the corresponding state-of-the-art methods. Furthermore, we have developed a repository with representative algorithms (https://github.com/DSE-MSU/DeepRobust/tree/master/deeprobust/graph). The repository enables us to conduct empirical studies to deepen our understandings on attacks and defenses on graphs.

==> tables/categ.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[ht]
\small
\begin{tabular}{@{}lllllll@{}}
\toprule
Attack Methods                                                                                             & \begin{tabular}[c]{@{}l@{}}Attack \\ Knowledge\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Targeted or\\ Untargeted\end{tabular} & \begin{tabular}[c]{@{}l@{}}Evasion or\\ Poisoning\end{tabular} & Perturbation Type                                                           & Application                                                                         & Victim Model                                                                 \\ \midrule
\begin{tabular}[c]{@{}l@{}}PGD, \\ Min-max~\cite{xu2019topology-attack}\end{tabular} & White-box                                                     & Untargeted                                                       & Both                                                           & Add/Delete edges                                                            & Node Classification                                                                 & GNN                                                                          \\
\cite{ig-attack}                                                                          & White-box                                                     & Both                                                             & evasion                                                        & Add/Delete edges                                                            & Node Classification                                                                 & GNN                                                                          \\
\cite{wang2019attacking-ccs}                                                              & \begin{tabular}[c]{@{}l@{}}White-box,\\ Gray-box\end{tabular} & Targeted                                                         & Poisoning                                                      & Add/Delete edges                                                            & Node Classification                                                                 & GNN                                                                          \\
Nettack~\cite{nettack}                                                               & Gray-box                                                      & Targeted                                                         & Both                                                           & \begin{tabular}[c]{@{}l@{}}Add/Delete edges,\\ Modify features\end{tabular} & Node Classification                                                                 & GNN                                                                          \\
Metattack~\cite{metattack}                                                           & Gray-box                                                      & Untargeted                                                       & Poisoning                                                      & Add/Delete edges                                                            & Node Classification                                                                 & GNN                                                                          \\
RL-S2V~\cite{rl-s2v}                                                                 & Black-box                                                     & Targeted                                                         & Evasion                                                        & Add/Delete edges                                                            & \begin{tabular}[c]{@{}l@{}}Graph classification,\\ Node Classification\end{tabular} & GNN                                                                          \\
ReWatt~\cite{rewatt}                                                                 & Black-box                                                     & Untargeted                                                       & Evasion                                                        & Add/Delete edges                                                            & Graph classification                                                                & GNN                                                                          \\
NIPA~\cite{nipa}                                                                     & Black-box                                                     & Untargeted                                                       & Poisoning                                                      & Inject nodes                                                                & Node Classification                                                                 & GNN                                                                          \\
\cite{node-embedding-poisoning}                                                           & Black-box                                                     & Both                                                             & Poisoning                                                      & Add/Delete edges                                                            & \begin{tabular}[c]{@{}l@{}}Node Classification, \\ Community Detection\end{tabular} & \begin{tabular}[c]{@{}l@{}}Network \\ Emebdding \\ Models\end{tabular}       \\
GF-Attack~\cite{gf-attack}                                                           & Black-box                                                     & Targeted                                                         & Poisoning                                                      & Add/Delete edges                                                            & Node Classification                                                                 & \begin{tabular}[c]{@{}l@{}}Network \\ Emebdding \\ Models\end{tabular}       \\
\cite{TowardsDP-knowledge-grap}                                                           & White-box                                                     & Targeted                                                         & Poisoning                                                      & Add/Delete facts                                                            & Plausibility Prediction                                                             & \begin{tabular}[c]{@{}l@{}}Knowledge \\ Graph \\ Embedding\end{tabular}      \\
\cite{liu2019unified-ssl}                                                                 & \begin{tabular}[c]{@{}l@{}}White-box,\\ Gray-box\end{tabular} & Untargted                                                        & Poisoning                                                      & Flip label                                                                  & \begin{tabular}[c]{@{}l@{}}Classification,\\ Regression\end{tabular}                & G-SSL                                                                        \\
CD-ATTACK~\cite{\{li2020adversarial-hiding-community}                                & Black-box                                                     & Targeted                                                         & Poisoning                                                      & Add/Delete edges                                                            & Community Detection                                                                 & \begin{tabular}[c]{@{}l@{}}Community \\ Detection \\ Algorithms\end{tabular} \\ \bottomrule
\end{tabular}
\end{table*}
